Stable Approximation Algorithms for the Dynamic Broadcast Range-Assignment Problem

Let $P$ be a set of points in $\mathbb{R}^d$, where each point $p\in P$ has an associated transmission range $\rho(p)$. The range assignment $\rho$ induces a directed communication graph $\mathcal{G}_{\rho}(P)$ on $P$, which contains an edge $(p,q)$ iff $|pq| \leq \rho(p)$. In the broadcast range-assignment problem, the goal is to assign the ranges such that $\mathcal{G}_{\rho}(P)$ contains an arborescence rooted at a designated node and whose cost $\sum_{p \in P} \rho(p)^2$ is minimized. We study trade-offs between the stability of the solution -- the number of ranges that are modified when a point is inserted into or deleted from $P$ -- and its approximation ratio. We introduce $k$-stable algorithms, which are algorithms that modify the range of at most $k$ points when they update the solution. We also introduce the concept of a stable approximation scheme (SAS). A SAS is an update algorithm that, for any given fixed parameter $\varepsilon>0$, is $k(\epsilon)$-stable and maintains a solution with approximation ratio $1+\varepsilon$, where the stability parameter $k(\varepsilon)$ only depends on $\varepsilon$ and not on the size of $P$. We study such trade-offs in three settings. - In $\mathbb{R}^1$, we present a SAS with $k(\varepsilon)=O(1/\varepsilon)$, which we show is tight in the worst case. We also present a 1-stable $(6+2\sqrt{5})$-approximation algorithm, a $2$-stable 2-approximation algorithm, and a $3$-stable $1.97$-approximation algorithm. - In $\mathbb{S}^1$ (where the underlying space is a circle) we prove that no SAS exists, even though an optimal solution can always be obtained by cutting the circle at an appropriate point and solving the resulting problem in $\mathbb{R}^1$. - In $\mathbb{R}^2$, we also prove that no SAS exists, and we present a $O(1)$-stable $O(1)$-approximation algorithm.

==> almost-maximally-stable-algorithms.tex <==
%--------------------------------------------------------------------------------------------
\section{1-Stable, 2-Stable, and 3-Stable Algorithms in $\Reals^1$}
\label{sec:max-stable}
%--------------------------------------------------------------------------------------------
\mdb{I suggest to omit this section, and only deal with 1-, 2- and 3-stable algorithms in the appendix.}
In the previous section we presented a $(2k+6)$-stable algorithm whose approximation ratio
is~$1+2^{\alpha}/k^{\alpha-1}$, which provided us with a SAS. For small~$k$ the algorithm
is not very good: the most stable algorithm we can get is 6-stable,
by setting~$k=0$. A more careful analysis shows that the approximation ratio
of this 6-stable algorithm is~3. In this section we study more stable algorithms.
We first present a 1-stable $O(1)$-approximation algorithm; obviously,
this is the best we can do in terms of stability. This algorithm can only
handle insertions. (Deletions would be 3-stable.)
We then present a straightforward 2-stable 2-approximation
algorithm. Finally, we show that it is possible
to get an approximation ratio strictly below~2 using a 3-stable algorithm; see Table~\ref{ta:stableresults} for an overview.
%In the appendix we also present (non-matching) lower bounds for 1-stable and 2-stable algorithms.
%
\begin{table}[h]
\begin{center}
\begin{tabular}{c||c|l} 
$\ell$-stable algorithm & Approximation Ratio  & Remarks  \\ 
\hline
$\ell=1$  & $6+2\sqrt{5}\approx10.47$   & $\alpha=2$, insertions only \\
$\ell=2$  & 2                           & for any $\alpha > 1$  \\
$\ell=3$  & 1.97                        & $\alpha = 2$  \\ 
\end{tabular}
\caption{An overview of the approximation ratio of 1-stable, 2-stable and 3-stable algorithms}
\label{ta:stableresults}
\end{center}
\end{table}


==> mst-update-lemma.tex <==

\subsection{Proof of Lemma~\ref{le:mst-update}}
\label{app:proof-of-mst-update}
%------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------
\begin{proof}
We prove the first part of the lemma, namely that be any MST $T$ on~$P$
can be converted into an MST $T'$ on $P' = P\cup\{q\}$ 
such that all edges in $T'$ that are not incident to $q$ also occur in~$T$.
The second part of the lemma, which states that the reverse is true
as well, can be proved in a similar way.

Let $E' := P' \times P'$ be the set of all potential MST edges in $T'$,
and define $E := P \times P$. Denote the length of an edge $e\in E'$ by $|e|$. 
We define an ordering~$\prec$ on~$E'$ such that $e \prec e’$ if 
(i) $|e| < |e’|$, or
(ii) $|e|=|e’|$ and $e$ was an edge in $T$ but $e’$ was not.
When $|e|=|e’|$ but case~(ii) does not apply, we order $e$ and $e’$ arbitrarily. 
Note that the ordering on $E'$ induces an ordering on $E$. 
We claim  that running Kruskal’s algorithm on $P$, with the edges handled in the 
order specified by~$\prec$, will produce $T$. 

We prove the claim by proving the following statement by induction on $i$:  the first $i$ edges in the $\prec$-ordering 
are added to the MST by Kruskal’s algorithm if and only if they are in~$T$. For $i=0$ the claim trivially holds,
so suppose $i>0$ and let $e$ be the $i$-th edge in the $\prec$-ordering. If the algorithm does not add $e$, then the 
addition of $e$ would have generated a cycle, which (by the induction hypothesis) implies that $e$ cannot be in $T$. 
If the algorithm adds~$e$, then $e$ must also be in $T$. Indeed, suppose for a contradiction that $e$ is not in $T$
and let $\Gamma$ be the cycle  created when adding $e$ to $T$. Then for any edge $e’\in\Gamma$ we have 
$|e’|\geq |e|$, otherwise $T$ cannot be optimal. But then $e’ \prec e$. By the induction hypothesis
this implies that all edges $e’\in\Gamma\setminus\{e\}$ (which are in $T$) have been added by the algorithm,
contradicting that the algorithm would add $e$.
\medskip

We now generate $T'$ by running Kruskal’s algorithm on $P'$, 
with the edges handled in the order specified by~$\prec$. We claim that $T'$ has the required properties.

Suppose for a contradiction that there is an edge in $T'$ that is not incident to $q$ and that does not occur in~$T$.
Let $e$ be the first such edge in the $\prec$-ordering. Let $E'(e)$ be the set of edges already added to $T'$ when 
$e$ is handled in the construction of $T'$, and let $E(e)$ be the set of edges already added to $T$ when $e$ is 
handled in the construction of $T$. Then  $E'(e)\cup\{e\}$ does not have a cycle, because $e$ was added to $T'$.
On the other hand, $E(e)\cup\{e\}$ contains a cycle, $\Gamma$, because $e$ was not added to $T$. 
Then, for any edge $e’\neq e$ in $\Gamma$ there must be a path in $E'(e)$ between the endpoints of~$e’$ , 
contradicting the fact that $E'(e)\cup\{e\}$ does not have a cycle and thus proving the lemma.
Indeed, if $e’\in E'(e)$ we trivially have a path, so assume this is not the case. Consider the moment
at which~$e’$ was handled
in the construction of $T'$. Then the addition of $e’$ would generate a cycle (otherwise it would have been added),
and so there is a path between the endpoints of~$e’$.
\end{proof}
%--------------------------------------------------------------------------------------
